Probing squeezing for gravitational-wave detectors with an audio-band field

Squeezed vacuum states are now employed in gravitational-wave interferometric detectors, enhancing their sensitivity and thus enabling richer astrophysical observations. In future observing runs, the detectors will incorporate a filter cavity to suppress quantum radiation pressure noise using frequency-dependent squeezing. Interferometers employing internal and external cavities decohere and degrade squeezing in complex new ways, which must be studied to achieve increasingly ambitious noise goals. This paper introduces an audio diagnostic field (ADF) to quickly and accurately characterize the frequency-dependent response and the transient perturbations of resonant optical systems to squeezed states. This analysis enables audio field injections to become a powerful tool to witness and optimize interactions such as inter-cavity mode matching within gravitational-wave instruments. To demonstrate, we present experimental results from using the audio field to characterize a 16 m prototype filter cavity.

==> ADF Paper/preamble.tex <==

\def\i{\mathrm{i}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Types

\newcommand{\review}[1]{\textcolor{magenta}{#1}}
\newcommand{\rough}[1]{\textcolor{gray}{#1}}
\newcommand{\psub}[1]{{\bf #1:}\\}

% disable some?
% \renewcommand{\psub}[1]{}   % comment this out to allow paragraph headings
% \renewcommand{\review}[1]{#1}  % comment this out to color text for review

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parameters

\newcommand{\VarWithSub}[2]{#1_{\mathrm{#2}}}

\def\Amat{\mathbf{A_2}}
\def\alphaFC{\VarWithSub{\alpha}{fc}}
\def\alphaAFC{\VarWithSub{\alpha}{afc}}
\def\Tin{\VarWithSub{T}{in}}
\def\lengthFC{\VarWithSub{L}{fc}}
\def\loss{\mathcal{L}}
\def\bZeta{\mathbf{b}_\zeta}
\def\gammaIfo{\VarWithSub{\gamma}{ifo}}
\def\gammaFC{\VarWithSub{\gamma}{fc}}
\def\gammaAFC{\VarWithSub{\gamma}{afc}}
\def\K{\mathcal{K}}
\def\Lambdaro{\VarWithSub{\Lambda}{ro}}
\def\Lambdainj{\VarWithSub{\Lambda}{inj}}
\def\omegaFC{\VarWithSub{\omega}{fc}}
\def\OmegaSQL{\VarWithSub{\Omega}{SQL}}
\def\phimm{\VarWithSub{\phi}{mm}}
\def\Rphi{\mathbf{R}_{\phi}}
\def\Rnphi{\mathbf{R}_{-\phi}}
\def\rhoFC{\VarWithSub{\rho}{fc}}
\def\rhoAFC{\VarWithSub{\rho}{afc}}
\def\rFC{\VarWithSub{r}{fc}}
\def\rAFC{\VarWithSub{r}{afc}}
\def\tmm{\VarWithSub{t}{mm}}
\def\tauInj{\VarWithSub{\tau}{inj}}
\def\tauM{\VarWithSub{\tau}{m}}
\def\tauRo{\VarWithSub{\tau}{ro}}
\newcommand{\T}[1]{\mathbf{T_{#1}}}
\def\Id{\mathbf{I}}

\newcommand{\greenWavelength}{\SI{532}{\nano\meter}}
\newcommand{\redWavelength}{\SI{1064}{\nano\meter}}

\newcommand{\cavityLength}{\SI{16}{\meter}}
\newcommand{\aplusLength}{\SI{300}{\meter}}

\newcommand{\armPower}{\SI{750}{\kilo\watt}}
\newcommand{\sqlFreq}{\SI{61.4}{\hertz}}
\newcommand{\ifoBandwidth}{\SI{429}{\hertz}}

\newcommand{\cavityBandwidth}{\SI{90}{\hertz}}
\newcommand{\CLFfreq}{\SI{8.9}{\mega\hertz}}
\newcommand{\CLFdoubledFreq}{\SI{17.8}{\mega\hertz}}
\newcommand{\RLFfreq}{\SI{9.3}{\mega\hertz}}

\newcommand{\diagDetuning}{\SI{1}{\kilo\hertz}}

\newcommand{\optimalLoss}{\SI{16}{ppm}}
\newcommand{\criticalLoss}{\SI{55}{ppm}}

\newcommand{\sqzLevel}{\SI{5}{\decibel}}
\newcommand{\asqzLevel}{\SI{9}{\decibel}}
\newcommand{\gensqzLevel}{\SI{11}{\decibel}}
\newcommand{\totalLoss}{21\%}


%from frequency dependent loss paper
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\hrms}{\ensuremath{h_{\text{rms}}}}
\newcommand{\htot}{\ensuremath{h_{\text{T}}}}

\newcommand{\FBW}{\ensuremath{f_{\text{bw}}}}
\newcommand{\rate}{\ensuremath{r}}
\newcommand{\msol}{\ensuremath{M_\odot}}
\newcommand{\omegaL}{\ensuremath{\nu}}



\newcommand{\E}[1]{
  \ensuremath{\mathrm{E}\!\left\{ #1 \right\}}
  }
\newcommand{\VAR}[1]{
  \ensuremath{\mathrm{VAR}\!\left\{ #1 \right\}}
  }
\newcommand{\COV}[1]{
  \ensuremath{\mathrm{COV}\!\left\{ #1 \right\}}
  }
\newcommand{\Tr}[1]{
  \ensuremath{\text{Tr}\left\{#1\right\}}
}

\newcommand{\stat}[1]{\ensuremath{\hat{#1}}}
\newcommand{\qhat}[1]{\ensuremath{\hat{#1}}}
\newcommand{\sqzOP}{\ensuremath{\qhat{\mathcal{S}}}}
\newcommand{\dispOP}{\ensuremath{\qhat{\mathcal{D}}}}
\newcommand{\bsOP}{\ensuremath{\qhat{\mathcal{B}}}}

% matrix and vector in quadrature basis
\newcommand{\Qmat}[1]{\ensuremath{\mathbbl{#1}}}
\newcommand{\Qvec}[1]{\overset{\raisebox{-2pt}{\text{\tiny$\bm\rightarrow$}}}{\mathbbl{#1}}}

% matrix and vector in sideband basis
\newcommand{\Smat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Svec}[1]{\ensuremath{{\mathbf{#1}}}}

\newcommand{\Marrow}[1]{\overset{\text{\tiny$\bm\leftrightarrow$}}{#1}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Marrowbbl}[1]{\overset{\raisebox{-1pt}{\text{\tiny$\bm\Leftrightarrow$}}}{#1}}
\newcommand{\Dmat}[1]{\ensuremath{\Marrowbbl{\mathbf{#1}}}}
\newcommand{\Mrarrowbbl}[1]{\overset{\raisebox{-1pt}{\text{\tiny$\bm\Rightarrow$}}}{#1}}
\newcommand{\Dvec}[1]{\ensuremath{\Mrarrowbbl{\mathbf{#1}}}}
\newcommand{\delay}{\ensuremath{L}}

\newcommand{\Psqz}{\ensuremath{\vec{E}_{\text{SQZ}}}}
%\newcommand{\Pread}{\ensuremath{\vec{E}_{\text{OMC}}}}
\newcommand{\Pread}{\ensuremath{\vec{\mathcal{P}_{2}}}}

\newcommand{\conj}[1]{\ensuremath{{#1}^*}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\MM}{\ensuremath{\Upsilon}}
\newcommand{\MMR}{\ensuremath{\Upsilon_{\text{R}}}}
\newcommand{\MMI}{\ensuremath{\Upsilon_{\text{I}}}}
\newcommand{\MMO}{\ensuremath{\Upsilon_{\text{O}}}}
\newcommand{\MMF}{\ensuremath{\Upsilon_{\text{F}}}}
\newcommand{\cMM}{\ensuremath{1{-}\MM}}
\newcommand{\cMMR}{\ensuremath{1{-}\MMR}}
\newcommand{\cMMI}{\ensuremath{1{-}\MMI}}
\newcommand{\cMMO}{\ensuremath{1{-}\MMO}}
\newcommand{\cMMF}{\ensuremath{1{-}\MMF}}

\newcommand{\LT}{\ensuremath{\Lambda_{\text{T}}}}
\newcommand{\ET}{\ensuremath{\eta_{\text{T}}}}
\newcommand{\LI}{\ensuremath{\Lambda_{\text{I}}}}
\newcommand{\LO}{\ensuremath{\Lambda_{\text{O}}}}

%\newcommand{\Ophi}{\ensuremath{\overline{\phi}}}
\newcommand{\Ophi}{\ensuremath{\phi}}
\newcommand{\phiRMS}{\ensuremath{\phi_{\text{rms}}}}
\newcommand{\phiRMSsq}{\ensuremath{\phi^2_{\text{rms}}}}

\newcommand{\thetaRMS}{\ensuremath{\theta_{\text{rms}}}}
\newcommand{\thetaRMSsq}{\ensuremath{\theta^2_{\text{rms}}}}

\newcommand{\QLO}{\ensuremath{\Qvec{v}^{\dagger}}}
\newcommand{\QLOa}{\ensuremath{\Qvec{v}}}
\newcommand{\SLO}{\ensuremath{\Svec{v}^{\dagger}}}
\newcommand{\SLOa}{\ensuremath{\Svec{v}}}
\newcommand{\DLO}{\ensuremath{\Dvec{v}^\dagger}}
\newcommand{\DLOa}{\ensuremath{\Dvec{v}}}

\newcommand{\Hloss}{\ensuremath{\Qmat{H}_{\text{loss}}}}

\newcommand{\Mq}{\ensuremath{m_q}}
\newcommand{\Mp}{\ensuremath{m_p}}
\newcommand{\cMp}{\ensuremath{\conj{m}_p}}

\newcommand{\sql}{\ensuremath{\text{sql}}}
\newcommand{\subI}{\ensuremath{\text{I}}}
\newcommand{\subO}{\ensuremath{\text{O}}}
\newcommand{\subR}{\ensuremath{\text{R}}}
\newcommand{\subFC}{\ensuremath{\text{FC}}}
\newcommand{\subfc}{\ensuremath{\text{fc}}}
\newcommand{\IRO}{\ensuremath{\text{IRO}}}

\newcommand{\subF}{\ensuremath{\text{F}}}

\newcommand{\adf}{\ensuremath{\text{a}}}
\newcommand{\adfs}{\ensuremath{\text{a}\downarrow}}
\newcommand{\adfa}{\ensuremath{\text{a}\uparrow}}
\newcommand{\clf}{\ensuremath{\text{c}}}
\newcommand{\rlf}{\ensuremath{\text{r}}}

\newcommand{\arm}{\ensuremath{\text{a}}}
\newcommand{\src}{\ensuremath{\text{s}}}
\newcommand{\Arm}{\ensuremath{\text{A}}}
\newcommand{\Src}{\ensuremath{\text{S}}}
\newcommand{\itm}{\ensuremath{\text{a}}}
\newcommand{\etm}{\ensuremath{\text{e}}}
\newcommand{\srm}{\ensuremath{\text{s}}}

\newcommand{\tfh}{\ensuremath{\mathfrak{h}}}
\newcommand{\tfr}{\ensuremath{\mathfrak{r}}}
\newcommand{\tfrH}{\ensuremath{\mathfrak{r}_{\text{hom}}}}

\newcommand{\udarrow}{\ensuremath{{\uparrow}\hspace{-0.4ex}{\downarrow}}}
\newcommand{\aADF}{\ensuremath{a}}
\newcommand{\ADFtoU}{\ensuremath{\Svec{a}^{\uparrow}}}
\newcommand{\ADFtoL}{\ensuremath{\Svec{a}^{\downarrow}}}
\newcommand{\ADFto}{\ensuremath{\Svec{a}^{\udarrow}}}

\newcommand{\ADFU}{\ensuremath{\Svec{d}^{\uparrow}}}
\newcommand{\ADFL}{\ensuremath{\Svec{d}^{\downarrow}}}
\newcommand{\ADF}{\ensuremath{\Svec{d}^{\udarrow}}}
\newcommand{\ADFnorm}{\ensuremath{\delta}}

\newcommand{\ADFUs}{\ensuremath{\Svec{d}^{\uparrow}_{s}}}
\newcommand{\ADFLs}{\ensuremath{\Svec{d}^{\downarrow}_{s}}}
\newcommand{\ADFUa}{\ensuremath{\Svec{d}^{\upparrow}_{a}}}
\newcommand{\ADFLa}{\ensuremath{\Svec{d}^{\downarrow}_{a}}}

\newcommand{\eLOU}{\ensuremath{e^{\uparrow}}}
\newcommand{\eLOL}{\ensuremath{e^{\downarrow}}}
\newcommand{\eLO}{\ensuremath{e^
{\udarrow}}}
\newcommand{\eLOr}{\ensuremath{e'^{\udarrow}}}
\newcommand{\eLOno}{\ensuremath{\overline{e}^{\udarrow}}}
\newcommand{\eLOnor}{\ensuremath{\overline{e}^{\udarrow}}}

\newcommand{\eLOUs}{\ensuremath{e'^{\uparrow}_{s}}} 
\newcommand{\eLOUsnp}{\ensuremath{e^{\uparrow}_{s}}} 
\newcommand{\eLOLs}{\ensuremath{e'^{\downarrow}_{s}}}
\newcommand{\eLOUa}{\ensuremath{e'^{\uparrow}_{a}}}
\newcommand{\eLOLa}{\ensuremath{e'^{\downarrow}_{a}}}



\newcommand{\eLOUn}{\ensuremath{\overline{e}^{\uparrow}}} 
\newcommand{\eLOLn}{\ensuremath{\overline{e}^{\downarrow}}}
\newcommand{\eLOUsn}{\ensuremath{\overline{e}^{\uparrow}_{s}}} 
\newcommand{\eLOLsn}{\ensuremath{\overline{e}^{\downarrow}_{s}}}
\newcommand{\eLOUan}{\ensuremath{\overline{e}^{\uparrow}_{a}}}
\newcommand{\eLOLan}{\ensuremath{\overline{e}^{\downarrow}_{a}}}

\newcommand{\Hopo}{\ensuremath{\Smat{H}_{\text{O}}}}
\newcommand{\Hopor}{\ensuremath{\Smat{H}'_{\text{O}}}}

\newcommand{\smu}{\ensuremath{{\,\mu}}}
\newcommand{\snu}{\ensuremath{{\,\nu}}}

\newcommand{\SQZint}{\ensuremath{z}}
\newcommand{\SQZcosh}{\ensuremath{\cosh{\SQZint}}}
\newcommand{\SQZsinh}{\ensuremath{\sinh{\SQZint}}}

\newcommand{\SQZcoshp}{\ensuremath{\cosh{Z}}}
\newcommand{\SQZsinhp}{\ensuremath{\sinh{Z}}}

\newcommand{\SQZcosht}{\ensuremath{\cosh(2\SQZint)}}
\newcommand{\SQZsinht}{\ensuremath{\sinh(2\SQZint)}}

\newcommand{\SQZcoshh}{\ensuremath{\cosh\Big(\frac{\SQZint}{2}\Big)}}
\newcommand{\SQZsinhh}{\ensuremath{\sinh\Big(\frac{\SQZint}{2}\Big)}}

\newcommand{\angPUMP}{\ensuremath{\psi}}
\newcommand{\angPUMPh}{\ensuremath{\psi}}
\newcommand{\angSQZ}{\ensuremath{\phi}}
\newcommand{\angADF}{\ensuremath{\Phi}}
\newcommand{\angLO}{\ensuremath{\zeta}}
\newcommand{\angDET}{\ensuremath{\Delta}}

\newcommand{\Msys}{\ensuremath{\mathbf{M_{\text{sys}}}}}
\newcommand{\epADF}{\ensuremath{e^+_{\text{ADF}}}}
\newcommand{\emADF}{\ensuremath{e^-_{\text{ADF}}}}

\newcommand{\mm}{\ensuremath{\eta_{\text{fc}}}}
\newcommand{\Hr}{\ensuremath{\Qmat{H}_{\text{R}}}}
\newcommand{\Hfc}{\ensuremath{\Qmat{H}_{\text{fc}}}}
\newcommand{\Hifo}{\ensuremath{\Qmat{H}_{\text{IFO}}}}
\newcommand{\rp}{\ensuremath{r_+}}
\newcommand{\rmin}{\ensuremath{r_-}}
\newcommand{\bR}{\ensuremath{\Smat{R}}}
\newcommand{\bA}{\ensuremath{\Smat{A}}}
\newcommand{\bAi}{\ensuremath{\Smat{A}^{-1}}}

\newcommand{\fdloss}{\ensuremath{\eta}}
\newcommand{\fdrot}{\ensuremath{\theta}}
\newcommand{\fddep}{\ensuremath{\Xi}}
\newcommand{\thcav}{\ensuremath{\mathbf{\Theta_{\textbf{cav}}}}}

\newcommand{\SQZdB}{\ensuremath{N_{\text{dB}}}}

\newcommand{\IFOk}{\ensuremath{\mathcal{K}}}
\newcommand{\IFOr}{\ensuremath{\mathfrak{r}}}
\newcommand{\IFOg}{\ensuremath{\gamma_A}}
\newcommand{\tA}{x}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 
